The X-ray Behavior of Two CVs: TT Ari and DP Leo

We present ROSAT PSPC observations of the nova-like, or intermediate polar, TT Ari and the eclipsing polar DP Leo. Observations of TT Ari were performed as part of a simultaneous multiwavelength campaign. The X-ray spectrum of TT Ari from ROSAT was combined with Ginga observations to suggest the presence of three distinct emission components: an optically thin plasma, a dominating bremsstrahlung continuum and one or more iron emission lines. Simultaneous and later IUE observations show modulation in the absorption component of the P Cygni-like CIV line on the spectroscopic period indicating a complex wind structure. Three eclipses were observed from the DP Leo system with intensity dips, not previously observed, occurring prior to each eclipse. The dips are interpreted as the eclipse of the main emission region by an accretion stream varying in impact position or stream shape with time. The DP Leo spectrum is well fit by either a 25 eV blackbody or a soft power law. No evidence exists for accretion onto the stronger magnetic pole and severe limits were placed upon the flux from any hard bremsstrahlung component. We constrained distances to this system based upon model fits to the data.

==> READMErc <==
%auto-ignore
This file contains information on the paper entitled 
"The X-ray Behavior of Two CVs: TT Ari and DP Leo"
by Craig Robinson and France Cordova.
It will appear in the conference proceedings entitled
"Interacting Binaries" (ed. Allen W. Shafter).

This paper is in LATEX format and uses the included
"paspconf.sty" as well as the encapulated
PostScript format style file "epsf.sty" (for use with Rokicki's PostScript
driver called dvips).  The "epsf.sty" file is available from SISSA if it
does not exist at your site.

The paper has a length of 14 pages and includes 10 PostScript
figures.  These figures are contained within the uuencoded compressed-tar
file and should have been unpacked at the same time as this file.

Once the uuencoded compressed-tar file is unpacked, the following 13
files should appear:

READMErc (this file)
paspconf.sty (required LATEX style file)
rc1.ps   rc3.ps   rc4b.ps  rc6.ps   rc8.ps
rc2.ps   rc4a.ps  rc5.ps   rc7.ps   rc9.ps (Figures)
rc.tex (main LATEX file)

To view the file without figures, comment out "\plotone", "\plottwo"
and "\plotfiddle" commands.

To execute, process the file "robcor.tex" through the LATEX program
(e.g., latex robcor) to create the .dvi file.  The figures may
be appropriately included by running this output file through
the dvips driver (e.g., dvips robcor.dvi).

Questions or comments should be directed to Craig Robinson at
robinson@astro.psu.edu or 814-863-4690.


